Embedding Lexical Features via Low-Rank Tensors

Modern NLP models rely heavily on engineered features, which often combine word and contextual information into complex lexical features. Such combination results in large numbers of features, which can lead to over-fitting. We present a new model that represents complex lexical features---comprised of parts for words, contextual information and labels---in a tensor that captures conjunction information among these parts. We apply low-rank tensor approximations to the corresponding parameter tensors to reduce the parameter space and improve prediction speed. Furthermore, we investigate two methods for handling features that include $n$-grams of mixed lengths. Our model achieves state-of-the-art results on tasks in relation extraction, PP-attachment, and preposition disambiguation.

==> Makefile <==
# Matt Gormley
# 
# Makefile for LaTeX and Bibtex.  Change the NAME and BIB parameters
# to be the name of the .tex and .bib files respectively.

NAME=naaclhlt2016
BIB=references

all: $(NAME).pdf

$(NAME).pdf: $(BIB).bib
	latexmk -outdir=build -auxdir=build -pdf -pvc $(NAME).tex

# Run latexmk and contiuously rebuild.
serve: $(BIB).bib
latexmk -outdir=build -auxdir=build -pdf -pvc $(NAME).tex

references-TEMP.bib: references-original.bib
	bibtool -r bibtool-resource.txt -i references-original.bib \
	 	| perl -ne "print if not /.*publisher.*Association for Computational Linguistics/" \
	 	| perl -ne "print if not /Citeseer/" \
	 	> references.bib

# Clean up the various extra files created by pdflatex
# and by AucTex in Aquamacs. 
clean:
	rm -f $(NAME).aux $(NAME).bbl $(NAME).blg $(NAME).log \
		$(NAME).rel $(NAME).toc $(NAME).synctex.gz \
		$(NAME).out $(NAME).pdf \
		$(NAME).fls $(NAME).fdb_latexmk \
		$(NAME).loa $(NAME).lof $(NAME).lot \
		 _region_.* *~
	rm -rf auto/
	rm -rf build/

# The phony targets ensure that this will run even if a file named
# clean or all is accidently created.
.PHONY: all
.PHONY: clean
.PHONY: serve


==> training.tex <==
\section{Training}
\label{sec:train}

% In this section, we describe our training procedure for the 

In order to scale to large training sets, we can optimize equation~\ref{eq:objective} with stochastic gradient descent (SGD).
However, the objective has rank constraints. Therefore after each update step in SGD, it requires an expensive proximal operation that enforces the constraints on the learned parameters.
This will make the SGD algorithm inefficient.

To deal with such problem, we first simplified the learning objective in equation~\ref{eq:objective} and get an equivalent unconstrained objective.
The key idea is to pre-set the sizes of all projection matrices $\bW_i$s, so for each $\bW_i^{r_i\times d_i}$ ($r_i$ $<$ $d_i$), the upper bound of its rank will be $r_i$, which can satisfy the constrains in equation~\ref{eq:objective}.
Therefore all the possible values of $\bW_i$ will satisfy the constrain.
%
% adopt a different approach and remove the constraints to simplify the learning objective; 
%The key idea is to pre-set the sizes of all $\bW$s of the model, therefore the upper bound of ranks of
%the learned model can be fixed. Then as long as this upper bound can satisfy the constrains, all
%the possible sets of parameters can be learned will satisfy the constrains.
%the low-rank approximation method of~\cite{socher-EtAl:2012:EMNLP-CoNLL}. 
In particular, for the 3-way Tucker-form approximation, where $\cT = g \times \bW_1 \times \bW_2 \times \bW_3$, if we set $\bW_i$ as a $r_i \times d_i$ matrix, and $g$ as a $r_1 \times r_2 \times r_3$ tensor, the rank of $\cT$ will be at most $(r_1, r_2, r_3)$ and the constraints are always satisfied. The same idea can be applied to the CP-form approximation by restricting each $\bW_i$ to be an $r \times d_i$ matrix. With these matrices with fixed sizes, the objective becomes:
%($g$ is fixed to superdiagonal tensor for CP-form):
\begin{align}
%&\underset{\small{g,\bW_{1,...,n}}}{\textrm{minimize}} \sum_{(\bx,y)\in \mathcal{D}} \ell(\bx,y;g, \bW_{1,...,n})& \textrm{(Tucker)} \nonumber\\
%&\underset{\small{\bW_{1,...,n}}}{\textrm{minimize}} \sum_{(\bx,y)\in \mathcal{D}} \ell(\bx,y; \bW_{1,...,n})& \textrm{(CP)}\\
\begin{aligned}
& \underset{\small{g,\{\bW_i\}}}{\textrm{minimize}} \sum_{(\bx,y)\in \mathcal{D}} \ell(\bx,y;\be, g, \{\bW_i^{r_i\times d_i}\})& \textrm{(Tucker)} \\
& \underset{\small{\{\bW_i\}}}{\textrm{minimize}} \sum_{(\bx,y)\in \mathcal{D}} \ell(\bx,y;\be, \{\bW_i^{r\times d_i}\})& \textrm{(CP)}
\end{aligned} \nonumber
%\text{(Tucker-form)} \nonumber\\
%{\textrm{max}}_{\bW_{1,...,n}} \sum_{(\bx,y)\in \mathcal{D}} \ell(s(F(\bx,y);\bW_{1,...,n})) \nonumber \\
%\text{ (CP-form)}
%{\sum_{(\bx,y)\in \mathcal{D}} \ell(y, \arg \min_{y'} {s} (F(\bx,y');\cT))}
%\label{eq:obj_uncons}
\end{align}

%By Mo: no need to talk about non-convexity
%Note that this optimization problem is still non-convex due to the
%interactions among the parameter matrices $\bW_i$s (and $g$ for Tucker case).
  
%\begin{align}
%%\maximize{\cT}{\sum_{(\bx,y)\in \mathcal{D}} \ell(y, \arg \min_{y'} {\cT} (F(\bx,y')))}
%\max_{\cT} {\sum_{(\bx,y)\in \mathcal{D}} \ell(y, \arg \min_{y'} {\cT} (F(\bx,y')))}
%%\label{eq:objective}
%\end{align}

%\subsection{An Equivalent Form of Scoring Function}
%For computational efficiency, we re-write the scoring function as follows. Let
%$\mathbf{f}^{(i)} = \sum_{\{lf|w_{lf} = w_i\}} f_{lf}$
%denote the unlexical parts associated with each word $w_i$. 
%Assume we have $T$ different words, the scoring function can be written as
%\begin{align}
%P(y|\bx;\cT) &\! \propto\! \exp\left \{ \sum_{i=1 }^T g \times_y \bh_y \times_f \bh_{\mathbf{f}^{(i)}} \times_w \bh_{w_i} \right \} \nonumber \\
%& \! \propto\! \exp\left \{ (g \times_y \bh_y)  \odot \left( \sum_{i=1}^T \bh_{\mathbf{f}^{(i)}} \otimes \bh_{w_i} \right) \right \}. 
%\label{eq:train-equivalent}
%\end{align}

% =======
%For computational efficiency, we can re-write the equation as follows:
%Denote $\mathbf{f}_{w_i} = \sum_{\{lf|w_{lf} = w_i\}} f_{lf}$, which is the unlexical parts associated with each word. Assume we have $T$ different words, we can re-write the equation as:
%\begin{align}
%&P(y|\bx;\cT) \propto \exp\left \{ \sum_{i=1 }^T g \times_y \bh_y \times_f \bh_{\mathbf{f}_{w_i}} \times_e \bh_{e_{w_i}} \right \} \nonumber \\
%&  = \exp\left \{ (g \times_y \bh_y)  \odot \left( \sum_{i=1}^T \bh_{\mathbf{f}_{w_i}} \otimes \bh_{e_{w_i}} \right) \right \}
%\label{eq:train-equivalent}
%>>>>>>> 8f2118e5e4ec37a5d875acbb75934e9e42937244

%\paragraph{Stochastic Gradient for Low-rank Tensors}
Now we can apply normal SGD on the above simplified objectives, and jointly optimize these projection matrices $\bW_i$s (and core tensor $g$ for Tucker case). 
Specifically, in this paper we update the parameters with AdaGrad \cite{duchi2011adaptive} and compute gradients via the chain-rule.
%Given the scoring function, we optimize the following log-likelihood objective with AdaGrad \cite{duchi2011adaptive} and compute gradients via back-propagation:
%\begin{align}
%\textstyle \mathcal{L}(g,\{\bW \}) = \frac{1}{|D|} \sum_{(y, \bx )\in D} \log P(y | \bx; g,\{\bW\}), \nonumber
%\vspace{-0.1 in}
%\end{align}
%where $D$ is the training set. 
See Appendix A for the detailed gradients.% for updating the parameters.
%For
%each instance $(y, \bx)$ we compute the gradient of the log-likelihood $\ell = \log P(y | \bx;
%g,\{\bW\})$. We define the vector 
%%$\mathbf s=\left[ \bW_ \bh_y\sum_i T_y \odot (\mathbf{g_i} \otimes e_{w_i}) \right]_{1\le y \le L}$, 
%$\bs$, where $\bs_{y'}= \left[ \sum_{i=1}^T g \times_y \bh_{y'} \times_f \bh_{\mathbf{f}^{(i)}} \times_w \bh_{w_i} \right]$, 
%which yields ${\partial \ell}/{\partial \mathbf s} =\left[ (
%    I[y=y']-P(y' | \bx; g,\{\bW\}) )
%\right]_{ y' \in L}^T, \nonumber$
%where the indicator function $I[z]$ equals to 1 if $z$
%is true and zero otherwise. 
%Taking the view of unlexical features as example, 
%we have the following stochastic gradients
%(see the full gradients in Appendix):
%
%\paragraph{\lrfcmt}
%\begin{align}
%\frac{\partial \ell}{\partial g} &= \left( \sum_{y'=1}^L \frac{\partial \ell}{\partial \bs_{y'}} \bh_{y'} \right) 
%\otimes \left(\sum_{i=1}^T \bh_{\mathbf{f}^{(i)}} \otimes \bh_{w_i} \right), \nonumber
%\end{align}
%and
%\begin{align}
%\frac{\partial \ell}{\partial \bW_f} &= \sum_{i=1}^T \frac{\partial \ell}{\partial \bh_{\mathbf{f}^{(i)}}} \frac{\partial \bh_{\mathbf{f}^{(i)}}}{\partial \bW_f} \nonumber\\
%&= \sum_{i=1}^T\sum_{y'} I[f \in \mathbf{f}^{(i)}] \frac{\partial \ell}{\partial \mathbf{s}_{y'}} \cdot g \times_l \bh_{y'} \times_{w} \bh_{w_i}. \nonumber
%\end{align}
%
%\paragraph{\lrfcmcp}
%\begin{align}
%\frac{\partial \ell}{\partial \bW_f} %&= \sum_{i=1}^n \frac{\partial \ell}{\partial \bh_f} \frac{\partial \bh_f}{\partial \bW_f} \nonumber\\
%&= \sum_{i=1}^T \sum_{y'} I[f \in \mathbf{f}^{(i)}] \frac{\partial \ell}{\partial \mathbf{s}_{y'}} \left( \bh_{y'} \odot \bh_{w_i} \right). \nonumber
%\end{align}
%
%\removed{
%\subsection{Stochastic Gradient for Low-rank Tensors}
%we optimize the following
%log-likelihood objective with AdaGrad
%\cite{duchi2011adaptive} and compute gradients via back-propagation:
%\begin{align}
%\textstyle \mathcal{L}(g,\{\bW \}) = \frac{1}{|D|} \sum_{(y, \bx )\in D} \log P(y | \bx; g,\{\bW\}), \nonumber
%\vspace{-0.1 in}
%\end{align}
%where $D$ is the training set. For
%each instance $(y, \bx)$ we compute the gradient of the log-likelihood $\ell = \log P(y | \bx;
%g,\{\bW\})$. We define the vector 
%%$\mathbf s=\left[ \bW_ \bh_y\sum_i T_y \odot (\mathbf{g_i} \otimes e_{w_i}) \right]_{1\le y \le L}$, 
%$\bs$, where $\bs_{y'}= \left[ \sum_{i=1}^T g \times_y \bh_{y'} \times_f \bh_{\mathbf{f}^{(i)}} \times_w \bh_{w_i} \right]$, 
%which yields ${\partial \ell}/{\partial \mathbf s} =\left[ (
%    I[y=y']-P(y' | \bx; g,\{\bW\}) )
%\right]_{ y' \in L}^T, \nonumber$
%%\begin{align}
%%  $\frac{\partial \ell}{\partial \mathbf s} =\left[ \left( I[y,1]-P(1
%%      | S; T,\mathbf{W}) \right), \left( I[y,2]-P(2 | S;
%%      T,\mathbf{W}) \right), ..., \left( I[y,L]-P(L | S;
%%      T,\mathbf{W}) \right) \right]^T, \nonumber$
%%\end{align}
%where the indicator function $I[x]$ equals to 1 if $x$
%is true and 0 otherwise. 
%%Denote $\mathbf {a_f} = \sum_{j=1}^t e_{w_{f,j}} \cdot  \mathbf W_j $. 
%Taking the view of unlexical features as example, 
%we have the following stochastic gradients
%(see the full gradients in Appendix):%, where $\circ$ is the tensor product:
%\paragraph{\lrfcmt}
%\begin{align}
%\frac{\partial \ell}{\partial g} &= \left( \sum_{y'=1}^L \frac{\partial \ell}{\partial \bs_{y'}} \bh_{y'} \right) 
%\otimes \left(\sum_{i=1}^T \bh_{\mathbf{f}^{(i)}} \otimes \bh_{w_i} \right), \nonumber
%\end{align}
%and
%\begin{align}
%\frac{\partial \ell}{\partial \bW_f} &= \sum_{i=1}^T \frac{\partial \ell}{\partial \bh_{\mathbf{f}^{(i)}}} \frac{\partial \bh_{\mathbf{f}^{(i)}}}{\partial \bW_f} \nonumber\\
%&= \sum_{i=1}^T\sum_{y'} I[f \in \mathbf{f}^{(i)}] \frac{\partial \ell}{\partial \mathbf{s}_{y'}} \cdot g \times_l \bh_{y'} \times_{w} \bh_{w_i} \nonumber
%\end{align}
%
%\paragraph{\lrfcmcp}
%\begin{align}
%\frac{\partial \ell}{\partial \bW_f} %&= \sum_{i=1}^n \frac{\partial \ell}{\partial \bh_f} \frac{\partial \bh_f}{\partial \bW_f} \nonumber\\
%&= \sum_{i=1}^T \sum_{y'} I[f \in \mathbf{f}^{(i)}] \frac{\partial \ell}{\partial \mathbf{s}_{y'}} \left( \bh_{y'} \odot \bh_{w_i} \right) \nonumber
%\end{align}
%}

%\begin{small}
%\begin{align}
%\frac{\partial \ell}{\partial T} = \frac{\partial \ell}{\partial \mathbf s} \otimes \sum_{i=1}^n  \mathbf g_{i} \otimes \mathbf e_{w_i},
%%\end{align}
%%and
%%\begin{align}
%\nonumber
%\end{align}
%\end{small}
%%where $\sigma'(\cdot)$ is the gradient for any activate function $\sigma(\cdot)$.
%%We can fine-tune the word embeddings with \fct\ with the
%%following equation:
%\vspace{-0.3 in}
%\begin{small}
%\begin{align}
%\frac{\partial \ell}{\partial \mathbf W_f} = \sum_{i=1}^n \frac{\partial \ell}{\partial \mathbf g_{i}}  \frac{\partial \mathbf g_{i}}{\partial \mathbf W_f} = \sum_{i=1}^n \left( T \circ \frac{\partial \ell}{\partial \mathbf s}  \circ  \mathbf e_{w_i}  \right) \otimes \mathbf{f_i}. \nonumber
%%\frac{\partial \ell}{\partial e_w} &= \sum_{i=1}^n \frac{\partial \ell}{\partial \mathbf h_{f_i}} \sum_{j=1}^t I[w_j= w]\frac{\partial \mathbf h_{f_i}}{\partial e_w} = \sum_{i=1}^n \left( T \circ  \mathbf g_{f_i} \circ   \frac{\partial \ell}{\partial \mathbf s} \right) \cdot \sum_{j=1}^t I[w_j= w] \sigma' (\mathbf a_{f_i,j})  \mathbf W_j . \nonumber
%\end{align}
%\end{small}
%\vspace{-0.1 in}

